PaRiS: Causally Consistent Transactions with Non-blocking Reads and Partial Replication

Geo-replicated data platforms are at the backbone of several large-scale online services. Transactional Causal Consistency (TCC) is an attractive consistency level for building such platforms. TCC avoids many anomalies of eventual consistency, eschews the synchronization costs of strong consistency, and supports interactive read-write transactions. Partial replication is another attractive design choice for building geo-replicated platforms, as it increases the storage capacity and reduces update propagation costs. This paper presents PaRiS, the first TCC system that supports partial replication and implements non-blocking parallel read operations, whose latency is paramount for the performance of read-intensive applications. PaRiS relies on a novel protocol to track dependencies, called Universal Stable Time (UST). By means of a lightweight background gossip process, UST identifies a snapshot of the data that has been installed by every DC in the system. Hence, transactions can consistently read from such a snapshot on any server in any replication site without having to block. Moreover, PaRiS requires only one timestamp to track dependencies and define transactional snapshots, thereby achieving resource efficiency and scalability. We evaluate PaRiS on a large-scale AWS deployment composed of up to 10 replication sites. We show that PaRiS scales well with the number of DCs and partitions, while being able to handle larger data-sets than existing solutions that assume full replication. We also demonstrate a performance gain of non-blocking reads vs. a blocking alternative (up to 1.47x higher throughput with 5.91x lower latency for read-dominated workloads and up to 1.46x higher throughput with 20.56x lower latency for write-heavy workloads).

==> sections/correctness.tex <==
\subsection{Correctness}
\label{sec:protocols:correctness}
We now provide an informal proof sketch that \ts{} provides causal consistency by showing that $i)$ reads observe a causally consistent snapshot and $ii)$ writes are atomic.

\begin{lemma}
\label{lemmas:1}
The snapshot time $sn_T$ of a transaction $T$ is always lower than the commit time of $T$, $sn_T < T.ct$.
\end{lemma}

\begin{proof}
Let $t$ be a transaction with snapshot time $sn_T$ and commit time $ct$. The snapshot time is determined during the start of the transaction (Alg. 2 Line 4). The commit time is calculated in the commit phase of the 2PC protocol, as maximum value of the proposed prepare times of all partitions participants in the transaction (Alg. 2 Line 34). In order to reflect causality when proposing a prepare timestamp, each partition proposes higher timestamp than the snapshot timestamp (Alg. 3 Lines 12). Thus, the commit time of a transaction, $ct$, is always greater than the snapshot time, $sn_T$.
\end{proof}


\begin{proposition}
\label{propositions:1}
If an update $u_2$ causally depends on an update $u_1$, $u_2\leadsto u_1$, then $u_1.ut < u_2.ut$.
\end{proposition}

\begin{proof}
Let $c$ be the client that wrote $u_2$. There are three cases upon which $u_2$ can depend on $u_1$, described in Section~\ref{sec:model:cc}: \textit{1}) $c$ committed $u_1$ in a previous transaction; \textit{2}) $c$ has read $u_1$, written in a previous transaction and \textit{3}) $c$ has read $u_3$, and there exists a chain of direct dependencies that lead from $u_1$ to $u_3$, i.e. $u2 \leadsto ... \leadsto u_3$ and $u_3 \leadsto u_1$. 

\textit{Case 1}. When a client commits a transaction, it piggybacks the last update transaction commit time $hwt_c$, if any, to its commit request for the transaction coordinator (Alg. 1 Line 27) which is, furthermore, piggybacked as $ht$ in its prepare requests to the involved partitions (Alg. 2 Line 31).
To reflect causality when proposing a commit timestamp, each partition proposes higher timestamp than both $ht$ and the snapshot timestamp (Alg. 2 Lines 10--13). The coordinator of the transaction chooses the maximum value from all proposed times from the participating partitions (Alg 2 Line 34) to serve as commit time, $ct$ for all the items in the transaction. The data item is written in the key-value store with $ct$ as its update time, $ut$ (Algorithm 3 Lines 3 and 11).
So, when $c$ commits the transaction that updates $u_2$, it piggybacks the commit time of the transaction that updated $u_1$ and from the discussion above it follows that $u_1.ct < u_2.ct$. Because the commit time of a transaction is the update time of all the data items versions (Alg. 4 Lines 2 and 13), we have $u_1.ut < u_2.ut$.

\textit{Case 2:} $c$ could have read $u_1$ either from $c$'s client cache or from the transaction causal snapshot $sn_T$. 

If $c$ has read $u_1$ from  $c$'s client cache, then $c$ has written $u_1$ either in a previous transaction in the same thread of execution or in the current one. If $c$ wrote $u_1$ in the same transaction where $u_2$ is also written, then it is not possible to have $u_2 \leadsto u_1$ because all the updates from that transaction will be given the same commit, i.e. update time and we will have $u_1.ut = u_2.ut$. Hence, $u_1$ must be written in a previous transaction and from \textit{Case 1} it follows that $u_1.ut < u_2.ut$.

Next, we will consider the case when $c$ read $u_1$ from the causal snapshot $sn_{T}$ that contains $u_1$.
When a transaction $T$ is started, the snapshot $sn_T$ is determined by Alg. 2 Line 2, $sn_T = max\{ust_c, ust_n^m\}$. From Alg. 3 Line 6 we have that $u_1.ut \leq ust = sn_T$. From Lemma~\ref{lemmas:1} it follows that $u_1.ut \leq sn_t < u_2.ct= u_2.ut$. Hence, $u1.ut < u_2.ut$

\textit{Case 3:}If $u_2$ depends on $u_1$ because of a transitive dependency out of $c's$ thread-of-execution, it means that there exists a chain of direct dependencies that lead from u2 to u3, i.e., $u2 \leadsto ... \leadsto u3$ and $u3 \leadsto u1$. Each pair in the transitive-chain, belongs to either  \textit{Case 1} or \textit{Case 2}. Hence, the proof of \textit{Case 3} comes down to chained application of the correctness arguments from \textit{Case 1} and \textit{Case 2}, proving that each element has an update time lower than its successor's.

\end{proof}

\begin{proposition}
\label{propositions:2}
A partition vector clock $VV_n^m[i] = t$ implies that $p_n^m$ has received all updates from $i-th$ replica with commit time, $ct \leq t$.
\end{proposition}
\begin{proof}
We need to show that this proposition is valid for both local and remote updates. To prove the former, we show that there are no pending local updates with commit timestamp $ct \leq t$. When $p_n^m$ updates the local replica vector clock entry $VV_n^m[r]$, it finds the minimum prepare timestamp of all transactions that are currently in the prepare phase (Alg 4. Line 6). Because the commit time is calculated as the maximum of all prepare times (Alg 2. Line 34) and the HLC clock is monotonic (Alg. 3 Lines 10 and 16), it is guaranteed that all future transactions will receive a commit time which is greater than or equal to this minimum prepare timestamp. So, when the $VV_n^m[r]$ is set to the minimum of the prepare times of all transactions in the prepare queue minus 1(Alg. 4 Line 6), $p_n^m$ has already received all updates for the snapshot $VV_n^m[i] = t$.

To show the latter, we use prove by contradiction. Assume there is a remote update $u$ from $i-th$ replica such that $u.ct < t$, and $p_m^n$ has not received $u$. By Alg. 3 Line 22, the partition would have received an update $u'$ such that $u'.ct = t$. The updates are sent in the order of their commit timestamps (Alg 4 Lines 9--15). Hence, if $u'.ct > u.ct$ the $p_n^m$ could not have received another update $u'$ before $u$. Therefore, $u.ct > t$, implying that $u.ct \nless t$, leading to the contradiction.
\end{proof}


\begin{proposition}
\label{propositions:3}
Snapshots in \ts{} are causal. 
\end{proposition}
\begin{proof} 
To start a transaction, a client $c$ piggybacks the freshest snapshot it has seen, ensuring the monotonicity of the snapshot seen by $c$ (Alg. 2 Lines 1–5). Commit timestamps reflect causality (Alg. 2 Line 19), and UST tracks a lower bound on the snapshot installed by every partition in all DCs (Alg. 4 Lines 34-38). If $X$ is within the snapshot of a transaction, so are its dependencies (Proposition ~\ref{propositions:1}). On top of the snapshot provided by the coordinator, the client applies its writes that are not in the snapshot. These writes cannot depend on items created by other clients that are outside the snapshot visible to $c$.
\end{proof}

\begin{proposition}
\label{propositions:4}
Writes are atomic.
\end{proposition}
\begin{proof}
Although updates are made visible independently on each partition $p_n^m$ involved in the commit phase, either all updates are made visible or none of them are, i.e. the atomicity is not violated. All updates from a transaction belong to the same snapshot because they all receive the same commit time (Alg 2 Lines 35). The updates are being installed in the order of their commit time (Alg. 4 Lines 9-20). The visibility of local and remote versions of items is determined by the transaction snapshot (Alg. 3 Lines 5), which is based on the value of $p_n^m$'s universal stable time $ust_n^m$ (Alg.1 Lines 2). $ust_n^m$ is computed by the UST protocol as the aggregate minimum of the version vectors entries of all partitions of all data centers (Alg.4 Lines 34-38).

\end{proof}

\ts{} implements TCC, as every transaction reads from a causally consistent snapshot (Proposition~\ref{propositions:3}) that includes all effects (Proposition~\ref{propositions:4}) of its causally dependent transactions.
